Learning Disentangled Semantic Spaces of Explanations via Invertible Neural Networks

Disentangled latent spaces usually have better semantic separability and geometrical properties, which leads to better interpretability and more controllable data generation. While this has been well investigated in Computer Vision, in tasks such as image disentanglement, in the NLP domain sentence disentanglement is still comparatively under-investigated. Most previous work have concentrated on disentangling task-specific generative factors, such as sentiment, within the context of style transfer. In this work, we focus on a more general form of sentence disentanglement, targeting the localised modification and control of more general sentence semantic features. To achieve this, we contribute to a novel notion of sentence semantic disentanglement and introduce a flow-based invertible neural network (INN) mechanism integrated with a transformer-based language Autoencoder (AE) in order to deliver latent spaces with better separability properties. Experimental results demonstrate that the model can conform the distributed latent space into a better semantically disentangled sentence space, leading to improved language interpretability and controlled generation when compared to the recent state-of-the-art language VAE models.

==> sections/limitations.tex <==
\section*{Limitations}
Despite the increased degree of separability and generation control achieved for the explanatory sentences by flow-based INNs, this work did not do any characterisation of of its suitability for broader controlled natural language inference tasks. How to achieve controlled, multi-hop natural language inference through this latent space with geometric properties still needs to be explored.

==> sections/qualitative.tex <==
\subsection{Qualitative Evaluation}
We analyse the representations of the trained models in terms of their disentanglement and composition, by applying three different techniques 1) traversals of the latent space, 2) latent space arithmetic, 3) encoding interpolation. %4) encoding visualization with dimensionality reduction.

\noindent
\textbf{Latent space traversals}
Traversal evaluation is a standard procedure with image disentanglement~\citep{higgins2016beta,kim2018disentangling}. The traversal of a latent factor is obtained as the decoding of the vectors corresponding to the latent variables, where the evaluated factor is changed within a fixed interval, while all others are kept fixed. If the representation is disentangled, when a latent factor is traversed, the decoded sentences should only change with respect to that factor. This means that after training the model we are able to probe the representation for each latent variable. In the experiment, the traversal is set up from a starting point given by a ``seed'' sentence. As illustrated in Table~\ref{tab:trav_examples} ...

\input{tables/trav_examples.tex}

% \noindent
% \textbf{Latent space arithmetic}
% In this experiment, the latent vectors for two sentences are added, subtracted or averaged, and then the resulting vectors are traversed. The sentence pairs are different by a single term, so that we can observe the latent variables affected by the change, and how they are affected. As illustrated in Table~\ref{tab:arith_examples}, ...

% \input{tables/arith_examples.tex}

\noindent
\textbf{Interpolation}
In this experiment, we demonstrate the ability of autoencoder models to provide smooth transition between latent space representations of sentences~\citep{bowman2016generating}. In practice, the interpolation mechanism takes two sentences $ x_1 $ and $ x_2 $, and uses their posterior mean as the latent features $ z_1 $ and $ z_2 $, respectively. It interpolates a path $ z_t = z_1 \cdot (1 - t) + z_2 \cdot t  $  with $ t $ increased from $ 0 $ to $ 1 $ by a step size of $ 0.1 $.  As a result, $ 9  $ sentences are generated on each interpolation step. In Table~\ref{tab:interpol_examples} we provide qualitative results with latent space interpolation on ...

\input{tables/interpol_examples.tex}

Based on those three experiments, the composition of such latent space could be conceptualised as in the projection illustrated in Figure~\ref{fig:latent_concept}.

\begin{figure}[ht]
    \centering
    % \includegraphics[scale=0.5]{figs/latent_diagram}
    \caption{Conceptualisation of a two-dimension cut of the latent space, applied to the first example in Table~\ref{tab:interpol_examples}.}
    \label{fig:latent_concept}
\end{figure}

\begin{figure}[t]
    % \includegraphics[scale=0.23]{figs/umap_all}
    \caption{UMAP plot of latent representations from Unsupervised VAE (U), DSR supervision (S) and Conditional VAE (C) (Top: LSTM, Bottom: Optimus).}
    \label{fig:umap}
\end{figure}

\paragraph{UMAP plot}
\textit{UMAP} (Uniform Manifold Approximation and Projection)~\cite{mcinnes2018umap} is a popular method for non-linear dimensionality reduction, that allows the visualization of complex high-dimensional feature spaces, such as the representation space produced by a VAE. Figure~\ref{fig:umap} presents a 2D plot of UMAP transformations for both baselines under three training frameworks, .... t-SNE transformations are also performed and the plots are presented in the supplemental material (Appendix~\ref{sec:apd_exp_res}).



==> tables/all_ds_by_exp.tex <==
%\documentclass[12pt]{article}
%\usepackage[a4paper, total={8.1in, 7in}]{geometry}
%\begin{document}
% \usepackage{booktabs}

% \begin{center}
\begin{table}[ht]
\scriptsize
\small
\centering
\setlength\tabcolsep{2.5pt}
% \resizebox{7.8cm}{!}{
\renewcommand\arraystretch{1}
\begin{tabular}{cccc}
\toprule
% \multicolumn{4}{c}{Optimus vs INN} \\ \hline
model & z-min-var $\downarrow$ & MIG  & Modularity \\ \hline
O(U)  & .451 & .027  & .758  \\ 
O(S)  & .453  & .067   & .753\\ 
O(C) & .401 & .039  & .751 \\
INN & \textbf{.350} & \textbf{.491} & \textbf{.844} \\ \hline
model & Disentanglement  & Completeness  & Informativeness $\downarrow$ \\ \hline
O(U) & \textbf{.307} & \textbf{.493}  & \textbf{.451}   \\ 
O(S) & .302  & .491 & .466     \\ 
O(C) & .306  & \textbf{.493} & .474   \\ 
INN & .186 & .270 & .503 \\ \toprule
\end{tabular}
% }
\caption{Disentanglement metrics. O(U), O(S), O(C) are three different training strategies for Optimus.} \label{tab:all_metrics}
\end{table}
% \end{center}



%\end{document}

% \begin{tabular}{ c|c|c |c}
% \toprule
% \multicolumn{5}{c}{Optimus vs INN} \\ \hline
% model & z-diff & z-min-var $\downarrow$ & MIG  & Modularity \\ \hline
% O(U) & .211 & .451 & .027  & .758  \\ \hline
% O(S) & \textbf{.254} & .453  & .067   & .753\\ \hline
% O(C) & .253 & .401 & .039  & .751 \\ \hline
% INN & .079 & \textbf{.350} & \textbf{.491} & \textbf{.844} \\ \hline
% model & Disentanglement  & Completeness  & Informativeness $\downarrow$ \\ \hline
% O(U) & \textbf{.307} & .493  & \textbf{.451}   \\ \hline
% O(S) & .302  & .491 & .466     \\ \hline
% O(C) & .306  & \textbf{.493} & .474   \\ \hline 
% INN & .186 & .270 & .503 \\ \toprule
% \end{tabular}

==> tables/animal_exp.tex <==
\begin{center}
\begin{table}[ht]
\scriptsize
\setlength\tabcolsep{2.5pt}
\resizebox{7.8cm}{!}{
% \renewcommand\arraystretch{1.3}
\begin{tabular}{c|c|c|c|c|c}
\toprule
\multicolumn{6}{c}{Animal: disentanglement metrics} \\ \hline

classifier & train & accuracy & precision & recall  & f1 score \\ \hline
\multirow{2}{*}{KNN} & O & 0.968 & 0.968 & 0.968  & 0.968 \\
 & U & 0.960 & 0.960 & 0.960  & 0.960 \\
 & C & \textbf{0.968} & \textbf{0.968} & \textbf{0.968}  & \textbf{0.968} \\ \hline
 
\multirow{2}{*}{NB} & O & 0.929 & 0.929 & 0.929  & 0.929 \\
& U & 0.915 & 0.915 & 0.915  & 0.915 \\
 & C & \textbf{0.940} & \textbf{0.940} & \textbf{0.940}  & \textbf{0.940} \\ \hline
 
\multirow{2}{*}{SVM} & O & 0.951 & 0.951 & 0.951  & 0.951 \\
& U & 0.931 & 0.931 & 0.931  & 0.931 \\
 & C & \textbf{0.952} & \textbf{0.952} & \textbf{0.952}  & \textbf{0.952} \\ \toprule
\end{tabular}
}

\caption{disentanglement of ARG0 between Optimus (O), unsupervised INN (U), and supervised INN (S) (KNN: k-neighbours, NB: naive bayes, SVM: support vector machine).} \label{tab:animal_exp}
\end{table}
\end{center}

==> tables/animal_inv_exp.tex <==
\begin{center}
\begin{table}[ht]
\scriptsize
\setlength\tabcolsep{2.5pt}
\resizebox{7.8cm}{!}{
% \renewcommand\arraystretch{1.3}
\begin{tabular}{c|c|c|c}
\toprule
\multicolumn{4}{c}{Animal: invertibility test (backward: $T'$)} \\ \hline
train & ARG0-animal & ARG1-animal & ARG2-animal \\ \hline
U & \textbf{0.99} & \textbf{0.99} & 0.90 \\ \hline
C & 0.97 & 0.96 & \textbf{0.92} \\ \toprule
\end{tabular}
}
\caption{Invertibility test for Animal.} \label{tab:animal_inv_exp}
\end{table}
\end{center}

==> tables/arg1_exp.tex <==

\begin{center}
\begin{table}[ht]
\scriptsize
\setlength\tabcolsep{2.5pt}
\resizebox{7.8cm}{!}{
% \renewcommand\arraystretch{1.3}
\begin{tabular}{c|c|c|c|c|c}
\toprule
\multicolumn{6}{c}{ARG1: disentanglement proxy metrics (forward: $T$)} \\ \hline

classifier & train & accuracy & precision & recall  & f1 score \\ \hline
\multirow{3}{*}{KNN} & O & 0.958 & 0.958 & 0.958  & 0.958 \\
 & U & 0.951 & 0.951 & 0.951  & 0.951 \\
 & C & \textbf{0.969} & \textbf{0.969} & \textbf{0.969}  & \textbf{0.969}  \\ \hline
 
\multirow{3}{*}{NB} & O & 0.907 & 0.907 & 0.907  & 0.907 \\
 & U & 0.926 & 0.926 & 0.926  & 0.926 \\
 & C & \textbf{0.956} & \textbf{0.956} & \textbf{0.956}  & \textbf{0.956} \\ \hline
 
\multirow{3}{*}{SVM} & O & 0.956 & 0.956 & 0.956  & 0.956 \\
& U & 0.953 & 0.953 & 0.953 & 0.953 \\
 & C & \textbf{0.958} & \textbf{0.958} & \textbf{0.958}  & \textbf{0.958} \\ \toprule
\end{tabular}
}

\caption{disentanglement of ARG1 between Optimus (O), unsupervised INN (U), and supervised INN (S) (KNN: k-neighbours, NB: naive bayes, SVM: support vector machine).} \label{tab:arg1_exp}
\end{table}
\end{center}

==> tables/arg1_inv_exp.tex <==
\begin{center}
\begin{table}[ht]
\scriptsize
\setlength\tabcolsep{2.5pt}
\resizebox{7.8cm}{!}{
% \renewcommand\arraystretch{1.3}
\begin{tabular}{c|c|c|c|c}
\toprule
\multicolumn{5}{c}{ARG1: invertibility test (backward: $T'$)} \\ \hline
train & ARG1-food & ARG1-oxygen & ARG1-sun & ARG1-water \\ \hline
U & \textbf{0.99} & \textbf{0.98} & 0.95 & 1.00 \\ \hline
C & 0.96 & 0.95 & \textbf{0.96} & \textbf{1.00} \\ \toprule
\end{tabular}
}
\caption{Invertibility test for ARG1 (U: unsupervised case, C: cluster supervised case).} \label{tab:arg1_inv_exp}
\end{table}
\end{center}

==> tables/arith_examples.tex <==

\begin{table}[ht!]
\begin{tcolorbox}[fontupper=\small, fontlower=\small, middle=0.3cm]

\underline{animals require food for survival} \\
\underline{animals require warmth for survival} \\

% dim03: \textcolor{blue}{animals} take nutrients \\
dim03: \textcolor{blue}{animals} require nutrients \\
% dim3: \textcolor{blue}{animals} require food \\
dim03: \textcolor{blue}{animals} require food for survival \\
dim03: \textcolor{blue}{animals} need nutrients to survive \\

% dim12: animal food contains nutrients \\
% dim12: \textcolor{blue}{animals} usually require water \\
% dim12: plants require water \\
% dim12: food requires oxygen for survival \\
% dim12: crops require oxygen for survival \\

% dim12: \textcolor{blue}{fish} require water for survival \\
dim12: \textcolor{red}{seaweed} contains water and nutrients \\
dim12: \textcolor{blue}{fish} contains water vapor for survival \\
dim12: \textcolor{red}{water} can stay unchanged in an atmosphere
% dim12: \textcolor{red}{warm - water} means water that has warm temperatures
% dim31: wood is attracted to light \\
% dim31: wood is formed by moving water \\
% dim31: wood chips are used for making magnetic objects \\
% dim31: metal in a jar means forming a solid \\
% dim31: anemia is a cause of death by anotrophs \\
% dim31: nails are an inherited characteristic \\
% dim31: wax is a kind of material that can be formed by chemical reaction \\
% dim31: moss is formed by absorbing solar energy \\
% dim31: a hurricane is formed by convection of air \\
% dim31: a flood is when heavy water moves large amounts of water \\
% \tcblower
% \underline{animals require food for survival} \\
% \underline{animals require warmth for survival} \\

% \textcolor{blue}{igneous rocks} are found under the soil \\
% \textcolor{blue}{quartz} is usually very small in size \\
% \textcolor{blue}{quartz} is formed by magma cooling \\
% % organic material is made of solid and liquid by reacting chemically \\
% \textcolor{blue}{quartz} is made of iron and zinc \\
% \textcolor{blue}{silica} is made of argon and argon \\
% \textcolor{blue}{sedimentary} is formed by lithosphere collapsing \\
% \textcolor{blue}{diamond} is a kind of solid that can not be heated \\
% \textcolor{blue}{quartz} is made of more graphite than granite \\
\end{tcolorbox}
\caption{Latent space arithmetic from INN where the first two sentences are the inputs.}
\label{tab:arith_examples}
\end{table}

==> tables/generation_traversal.tex <==
% \begin{center} , title=Guided generation via decision tree
\begin{table}[h]
\begin{tcolorbox}[fontupper=\small, fontlower=\small]
\underline{Input: an animal needs food to thrive} \\ \\
dim14: \textcolor{blue}{an animal} requires food for survival \\
dim13: \textcolor{blue}{a living thing} requires food for survival \\
dim25: \textcolor{blue}{something} that is moist can protect a animal \\ 
% dim14: \textcolor{blue}{something} that an animal eats can be a source of food \\
dim02: \textcolor{blue}{something} harmful can cause an animal to be dead \\
dim14: \textcolor{blue}{something} that an animal eats has a positive impact on that animal \\
% dim00: \textcolor{blue}{something} that is a living thing is a source of something \\
dim05: \textcolor{blue}{something} to be a good thing has a positive impact on an environment
% dim24: \textcolor{blue}{something} that an animal eats is a good resource
\end{tcolorbox}
\caption{Guided generation from \textit{ARG0-animal} to \textit{ARG0-something} via decision tree.}
\label{tab:guide_generate}
\end{table}

==> tables/generative_factors_explanation.tex <==
% \begin{table*}[ht!]
% \scriptsize
% \begin{center}
% \begin{tikzpicture}
% \node (table) [inner sep=.1pt] {

\begin{table}[ht!]
%     \small \setlength\tabcolsep{4.5pt}
    \scriptsize
    \centering
\renewcommand\arraystretch{1.3}
    \begin{tabular}{|c|c|}  \hline
        \textbf{Generative Factors}         & \textbf{Semantic Roles}                       \\ \hline
        direction &  ARGM-DIR \\ \hline
        cause & ARGM-CAU \\ \hline
        purpose & ARGM-PRP \\ \hline
        more & ARGM-EXT \\ \hline
        location & ARGM-LOC \\ \hline
        argument & ARG0, ARG1, ARG2, ARG3, ARG4 \\ \hline
        manner & ARGM-MNR \\ \hline
        verb & ARGM-MOD, V \\ \hline
        goal & ARGM-GOL, ARGM-PRD, ARGM-PNC \\ \hline
        negation & ARGM-NEG \\ \hline
        if-then & ARGM-ADV, ARGM-DIS \\ \hline
        time & ARGM-TMP \\ \hline
        c-arg & C-ARG0, C-ARG1, C-ARG2, C-ARG3  \\ \hline
    \end{tabular}
    \caption{Generative factors for explanations.} 
    \label{tab:gen_fac_exp}
\end{table}

==> tables/interpol_examples.tex <==
%\documentclass[border=.1mm,tikz,preview]{article}
%
%\usepackage{tikz}
%\usepackage{xcolor}
%\usepackage{graphicx}
%\usepackage{multirow}
%\usetikzlibrary{positioning}
%
%\begin{document}

\begin{table}[ht!]
% \scriptsize
% \begin{center}
% \begin{tikzpicture}
% \node (table) [inner sep=.1pt] {
% \renewcommand\arraystretch{20}
% \begin{tabular}{p{0.3cm} p{6.3cm}}
% \setlength\tabcolsep{.5pt}
% \multirow{12}{*}{\rotatebox[origin=c]{90}{DSR Optimus}}
% & \textcolor{blue}{protons are found in the nucleus of an atom} \\
% & 1 protons are found in the nucleus of an atom \\
% & 2 1 atom is positive 1 in electric charge \\
% & 3 1 in 6000 is equal to 27 in 10 years \\
% & 4 if protons and neutrons have the same number of neutrons then those two particles are physically closer than one another \\
% & 5 if a neutron has a negative -10 electric charge then the atom will not be able to move \\
% & 6 if a neutron has a negative -10 electric charge then the neutron will not have a positive electric charge \\
% & \textcolor{blue}{if a neutral atom loses an electron then an atom with a positive charge will be formed} \\

% \end{tabular}
% };
% \draw [rounded corners=.5em, line width=.5pt] (table.north west) rectangle (table.south east);
% \end{tikzpicture}
% \end{center}
\begin{tcolorbox}[fontupper=\small, fontlower=\small, title=interpolation control: \textit{predicate-require}]
% \begin{enumerate}
% \end{enumerate}
% \textcolor{blue}{humans eat seeds} \\
% 1. humans eat fruits \\
% 2. humans eat seeds \\
% 3. humans eat insects \\ 
% 4. humans eat meat \\
% 5. humans eat plants \\
% 6. some animals eat prey \\
% 7. some animals must eat to survive \\
% 8. some animals must hunt for food \\
% 9. some animals must hunt their prey to survive \\
% \textcolor{blue}{some animals must hunt to survive}
\underline{source: humans \textcolor{blue}{require} freshwater for survival}\\
1. nonhumans \textcolor{blue}{require} water to survive \\
2. marine animals \textcolor{blue}{require} food for survival  \\
3. animals \textcolor{red}{must breath} to survive  \\
4. animals \textcolor{blue}{require} water for survival \\
5. animals \textcolor{blue}{require} water from their ecosystems  \\
6. animals \textcolor{blue}{require} water for survival \\
7. animals \textcolor{red}{must eat} food for survival \\
8. animals \textcolor{blue}{require} food for survival \\
9. animals \textcolor{blue}{require} food for survival \\
10. animals \textcolor{blue}{require} food for survival \\
\underline{target: animals \textcolor{blue}{require} food to survive}
\end{tcolorbox}

\caption{Interpolation examples (unsupervised INN).}
\label{tab:interpol_examples}
\end{table}

%\end{document}

==> tables/optimus_def_examples.tex <==

\begin{table}[ht!]
\begin{tcolorbox}[fontupper=\small, fontlower=\small, middle=0.3cm, title=ADD and SUB arithmetic]
ARGUMENT1: \\
\underline{a needle is a kind of object} \\
\underline{a tire is a kind of object} \\
\\
a wire \textcolor{blue}{is a kind of object} \\
a stick \textcolor{blue}{is a kind of object} \\
a ball \textcolor{blue}{is a kind of object} \\
% a hammer \textcolor{blue}{is a kind of object} \\
% a spoon \textcolor{blue}{is a kind of object} \\
 \\
a serotype is \textcolor{red}{similar to intersex egg} \\
a zygote contains \textcolor{red}{many cell types} \\
an xylem is made \textcolor{red}{of two clumps} \\
\\
VERB: \\
\underline{chromosomes are located in the cells} \\
\underline{Australia is located in the southern hemisphere} \\
\\
stars are \textcolor{blue}{located} in the solar system \\
Jupiter is \textcolor{blue}{located} in the milky way galaxy \\
aurora is \textcolor{blue}{located} in the constellation of Leo \\
% galaxies are \textcolor{blue}{located} on the outer planets \\
% Saturn is \textcolor{blue}{located} between the Sun and the Moon \\
\\
a crystal is \textcolor{red}{made} of metal \\
an alloy is \textcolor{red}{made} of iron and zinc \\
an aluminum plug \textcolor{red}{is} nonmagnetic \\
\\
LOCATION: \\
\underline{volcanoes are often found under oceans} \\
\underline{mosquitos can sense carbon dioxide in the air} \\
\\
polar ice sheets are located \textcolor{blue}{along rivers} \\
hurricanes occur frequently along the coast \textcolor{blue}{in Africa} \\
tide waves cause flooding \textcolor{blue}{in coastal waters} \\
% glacial ice caps are found \textcolor{blue}{in the South Pole} \\
% ice caps are located \textcolor{blue}{in the northern hemisphere} \\
\\
\textcolor{red}{valley is a kind of location} \\
\textcolor{red}{shape is a property of rocks} \\
\textcolor{red}{desert is a kind of place} \\
\\
TEMPORAL: \\
\underline{as the population of prey decreases competition} \underline{between predators will increase} \\
\underline{as competition for resources decreases the ability} \underline{to compete for resources will increase} \\
\\
\textcolor{blue}{as the population of an environment decreases} ecosystem function will decrease \\
\textcolor{blue}{as the spread of available air mass increases} the population will increase \\
\textcolor{blue}{as the number of heavy traffic required increases} the traffic cycle will decrease \\
% \textcolor{blue}{as population of an area increases} the average amount of land area will increase \\
\\
\textcolor{red}{some types of lizards live in water} \\
\textcolor{red}{a rose is rich in potassium} \\
\textcolor{red}{a fern grass roots foot trait means a fern grass} \\
\\
NEGATION: \\
\underline{pluto has not cleared its orbit} \\
\underline{sound can not travel through a vacuum} \\
\\
radio waves \textcolor{blue}{don't} have electric charge \\
electromagnetic radiation \textcolor{blue}{does not} have a neutral electric charge \\
electromagnetic radiation contains \textcolor{blue}{no} electric charge \\
% radio frequency is \textcolor{blue}{not} a static electromagnetic wave \\
% infrared radiation has \textcolor{blue}{no} frequency \\
\\
Mars \textcolor{red}{is} a kind of moon / planet \\
Anothermic rock \textcolor{red}{is} a kind of metamorphic rock \\
Anal Cetus's skeleton \textcolor{red}{is} a kind of fossil \\
% Anhecete \textcolor{red}{is} a kind of biothere \\
\end{tcolorbox}
\caption{Latent sapce arithmetic for five semantic tags.}
\label{tab:arith_other_examples}
\end{table}

==> tables/rec_examples1.tex <==
% \begin{table*}[ht!]
% \scriptsize
% \begin{center}
% \begin{tikzpicture}
% \node (table) [inner sep=.1pt] {

\begin{table*}[ht!]
    % \resizebox{\textwidth}{15mm}{
% \begin{tikzpicture}
    % \scriptsize
    \small
    \centering
\renewcommand\arraystretch{1.1}
    \begin{tabular}{p{5cm}p{5cm}p{5cm}}  \toprule
        \textbf{Explanations} & \textbf{BERT-GPT2} & \textbf{unsupervised INN} \\ \hline
        a fish is a kind of organism  & a fish is a kind of organism  & a fish is a kind of organism  \\ \hline
        a galaxy is a kind of celestial body & a galaxy is a kind of celestial body & a galaxy is a kind of celestial body \\ \hline
        water is the solvent & water is the solute & water is the solvent \\ \hline
        metal fork is made of metal for eating & metal fork is made of metal and usually made of metal & metal fork is made of metal for cooking \\ \hline
        to carry something means to contain something & to carry something means to bring something & to carry something means to transport that something \\ \hline
        a tape measure is a kind of tool for ( measuring distance ; measuring length ) & a tape measure is a kind of tool for measuring ( length ; distance ) & a scale is a kind of tool for measuring weight / length \\ \hline
        riding something is a kind of movement & walking is a kind of moving & riding is a kind of movement \\ \hline
        if a living thing is destroyed then the resources used by that living thing will become available & if something is dead then that something can rest in the environment & if a living thing is destroyed then the resources it uses will be available \\ \hline
        The chemical symbol for argon is Ar  & The chemical symbol for argon is Ar & The chemical symbol for argon is Ar \\ \hline
        exercise has a positive impact on a the strength of a body & strength has a positive impact on a human's survival & strength has a positive impact on a person's health \\ \hline
        laying eggs is a kind of property of an animal & laying an egg is a kind of inherited characteristic in birds & laying eggs is a kind of adaptation for reproducing \\ \hline
        bears eat berries ; insects ; animals & bears eat berries / insects / animals / food & bears eat berries / insects / animals / berries \\ \hline
        pollutants have a negative impact on the ( environment ; air quality ) & pollution has a negative impact on the ( environment ; the environment's water quality ; the environment's resources & pollution has a negative impact on the ( environment ; human health ) \\ \hline
        if an object touches something then one is exposed to that something & if an object touches something then one is exposed to that something & if an object touches something then one is exposed to that something \\ \hline
        a stopwatch is a kind of tool for measuring time & a stopwatch is a kind of tool for measuring time & a stopwatch is a kind of tool for measuring time \\ \toprule
    \end{tabular}
    \caption{Explanation reconstruction (left: original explanations from WorldTree corpus, middle: explanations from AutoEncoder, right: explanations from unsupervised INN).} 
    \label{tab:unsup_rec_explain}
\end{table*}

==> tables/stats_role.tex <==
\begin{center}
\begin{table*}[ht]
\scriptsize
\centering
\setlength\tabcolsep{2.5pt}
\resizebox{7.8cm}{!}{
\renewcommand\arraystretch{1.3}
\begin{tabular}{cccccc}
\toprule
\textbf{V} & \textbf{ARG0}& \textbf{ARG1}& \textbf{ARG2}  & \textbf{ARG3} & \textbf{ARG4} \\ \hline
1.000 & 0.320 & 0.985 & 0.609  & 0.006  & 0.001 \\ \hline
\textbf{ARGM-MOD} & \textbf{ARGM-DIR} & \textbf{ARGM-ADV} & \textbf{ARGM-PRP} & \textbf{ARGM-TMP} & \textbf{ARGM-LOC} \\ \hline
0.098 & 0.008 & 0.067  & 0.013  & 0.070 & 0.045 \\ \hline
\textbf{ARGM-GOL} & \textbf{ARGM-NEG} & \textbf{ARGM-MNR} & \textbf{ARGM-PRD} & \textbf{ARGM-DIS} & \textbf{ARGM-EXT} \\ \hline
0.002 & 0.012 & 0.020 & 0.002  & .0007 & .0004 \\ \hline
\textbf{ARGM-CAU} & \textbf{ARGM-PNC} & &  &  &  \\ \hline
.0005 & 0.0008  &  &  &  &  \\ \toprule
\end{tabular}
}
\caption{Count of semantic tags in explanations} \label{tab:stats_roles}
\end{table*}
\end{center}

==> tables/trav_examples.tex <==
% traversals results

\begin{table}[ht!]
\begin{tcolorbox}[fontupper=\small, fontlower=\small, middle=0.3cm]
\underline{some animals must hunt to survive} \\ \\
% dim01: \textcolor{blue}{some animals} must hunt to survive \\
dim01: \textcolor{blue}{some animals} must hunt for food \\
dim01: \textcolor{blue}{some animals} must hunt prey to survive \\
dim01: \textcolor{blue}{some animals} need to hunt to survive \\
% dim01: \textcolor{blue}{some animals} must hunt to survive \\

% dim01: \textcolor{blue}{some predators} prey animals must catch a large amount of prey 
% dim12: \textcolor{blue}{a mammal} requires fins to catch prey \\
dim12: \textcolor{blue}{an animal} needs to breathe to survive \\
dim12: \textcolor{blue}{an animal} can fly without air \\
dim12: \textcolor{blue}{a predator} must hunt to survive
% dim12: \textcolor{blue}{a predator} usually kills new organisms 
% dim12: if \textcolor{blue}{an animal} lives in an environment then there is more food available
% dim31: nails are made of proteins \\
% dim31: moss is a property of fungi \\
% dim31: carpet is made of particles in an airtight container \\
% dim31: a hurricane is formed by thermal conduction of particles \\
% dim31: a decrease in moisture is when warm air mass passes over a colder air \\
\end{tcolorbox}
\caption{Traversals showing \textcolor{blue}{held} semantic factors in explanations (unsupervised INN model).}
\label{tab:trav_examples}
\end{table}

==> tables/v_exp.tex <==

\begin{center}
\begin{table}[ht]
\scriptsize
\setlength\tabcolsep{2.5pt}
\resizebox{7.8cm}{!}{
% \renewcommand\arraystretch{1.3}
\begin{tabular}{c|c|c|c|c|c}
\toprule
\multicolumn{6}{c}{PRED: disentanglement metrics} \\ \hline

classifier & train & accuracy & precision & recall  & f1 score \\ \hline
\multirow{3}{*}{KNN}  & O & 0.964 & 0.964 & 0.964  & 0.964 \\
& U & 0.959 & 0.959 & 0.959  & 0.959 \\ 
& C & \textbf{0.972} & \textbf{0.972} & \textbf{0.972}  & \textbf{0.972} \\ \hline
 
\multirow{3}{*}{NB}  & O & 0.923 & 0.923 & 0.923  & 0.923 \\
& U & 0.927 & 0.927 & 0.927  & 0.927 \\ 
& C & \textbf{0.951} & \textbf{0.951} & \textbf{0.951}  & \textbf{0.951}  \\ \hline
 
\multirow{3}{*}{SVM}  & O & 0.956 & 0.956 & 0.956  & 0.956 \\
 & U & 0.950 & 0.950 & 0.950  & 0.950 \\ 
 & C & \textbf{0.958} & \textbf{0.958} & \textbf{0.958}  & \textbf{0.958} \\ \toprule
\end{tabular}
}

\caption{disentanglement of ARG0 between Optimus (O), unsupervised INN (U), and supervised INN (S) (KNN: k-neighbours, NB: naive bayes, SVM: support vector machine).} \label{tab:v_exp}
\end{table}
\end{center}

==> tables/v_inv_exp.tex <==
\begin{center}
\begin{table}[ht]
\scriptsize
\setlength\tabcolsep{2.5pt}
\resizebox{7.8cm}{!}{
% \renewcommand\arraystretch{1.3}
\begin{tabular}{c|c|c|c|c}
\toprule
\multicolumn{5}{c}{PRED: invertibility test (backward: $T'$)} \\ \hline
train & PRED-is & PRED-are & PRED-cause & PRED-require \\ \hline
U & 1.00 & \textbf{0.95} & 0.97 & 0.80 \\ \hline
C & \textbf{1.00} & 0.88 & 0.90 & \textbf{0.82} \\ \toprule
\end{tabular}
}
\caption{Invertibility test for PRED (U: unsupervised case, C: cluster supervised case).} \label{tab:arg1_inv_exp}
\end{table}
\end{center}
